Focus-to-Perceive Representation Learning: A Cognition-Inspired Hierarchical Framework for Endoscopic Video Analysis

Endoscopic video analysis is essential for early gastrointestinal screening but remains hindered by limited high-quality annotations. While self-supervised video pre-training shows promise, existing methods developed for natural videos prioritize dense spatio-temporal modeling and exhibit motion bias, overlooking the static, structured semantics critical to clinical decision-making. To address this challenge, we propose Focus-to-Perceive Representation Learning (FPRL), a cognition-inspired hierarchical framework that emulates clinical examination. FPRL first focuses on intra-frame lesion-centric regions to learn static semantics, and then perceives their evolution across frames to model contextual semantics. To achieve this, FPRL employs a hierarchical semantic modeling mechanism that explicitly distinguishes and collaboratively learns both types of semantics. Specifically, it begins by capturing static semantics via teacher-prior adaptive masking (TPAM) combined with multi-view sparse sampling. This approach mitigates redundant temporal dependencies and enables the model to concentrate on lesion-related local semantics. Following this, contextual semantics are derived through cross-view masked feature completion (CVMFC) and attention-guided temporal prediction (AGTP). These processes establish cross-view correspondences and effectively model structured inter-frame evolution, thereby reinforcing temporal semantic continuity while preserving global contextual integrity. Extensive experiments on 11 endoscopic video datasets show that FPRL achieves superior performance across diverse downstream tasks, demonstrating its effectiveness in endoscopic video representation learning. The code is available at https://github.com/MLMIP/FPRL.

==> sec/0_abstract.tex <==
\begin{abstract}

Endoscopic video analysis is crucial for early gastrointestinal screening, but its progress is constrained by limited high-quality annotations. While self-supervised video pre-training shows promise, existing methods designed for natural videos tend to prioritize dense spatio-temporal modeling and exhibit motion bias, neglecting the static, structured semantics that are critical for clinical decision-making. To address this challenge, we propose \textbf{F}ocus-to-\textbf{P}erceive \textbf{R}epresentation \textbf{L}earning (\textbf{FPRL}), a cognition-inspired hierarchical framework that emulates the clinical examination process of endoscopic videos. FPRL first focuses on intra-frame lesion-centric regions to learn static semantics, and then perceives their evolution across frames to model contextual semantics. To achieve this, FPRL employs a hierarchical semantic modeling mechanism that explicitly distinguishes and collaboratively learns both types of semantics. Specifically, it begins by capturing static semantics through the application of teacher-prior adaptive masking (TPAM) combined with multi-view sparse sampling. This approach mitigates redundant temporal dependencies and enables the model to concentrate on lesion-related local semantics. Following this, contextual semantics are derived through cross-view masked feature completion (CVMFC) and attention-guided temporal prediction (AGTP). These processes establish cross-view correspondences and effectively model structured inter-frame evolution, thereby reinforcing temporal semantic continuity while preserving global contextual integrity. Extensive experiments on 11 endoscopic video datasets show that FPRL achieves state-of-the-art performance across diverse downstream tasks, demonstrating its effectiveness and strong generalization in endoscopic video representation learning.


\end{abstract}

==> sec/1_introduction.tex <==
\section{Introduction}
\label{sec:introduction}


\begin{figure}[t]
    \centering
    \includegraphics[width=1\linewidth]{intro.png}
    \caption{(a) Dense spatio-temporal modeling often captures irrelevant semantics due to motion reliance. (b) Our hierarchical approach isolates static from dynamic context, extracting appearance features required for diagnosis.}
    \label{fig:introfig}
\end{figure}

% Endoscopic video analysis plays a vital role in the early screening and diagnosis of gastrointestinal diseases, but its development is severely limited by the scarcity of high-quality annotated data. To overcome this limitation, a straightforward approach is to leverage the successful experience from general video understanding to learn generalizable representations from large-scale unlabeled videos through self-supervised video pre-training \cite{tong2022videomae,bertasius2021spaceTimesformer,wang2023videomaev2}. Such methods design pretext tasks (\textit{e.g.}, frame reconstruction, temporal prediction, or masked completion) to capture spatio-temporal consistency without human annotations, thereby effectively alleviating the problem of annotation scarcity.    
% Endoscopic video analysis plays a vital role in the early screening and diagnosis of gastrointestinal diseases by enabling more accurate lesion detection and assisting clinicians in making timely decisions. However, its further development is severely constrained by the scarcity of high-quality annotated data, which limits the performance and generalization of current algorithms. To address this challenge, a natural strategy is to draw on advances in general video understanding and learn generalizable representations from large-scale unlabeled videos via self-supervised video pre-training \cite{tong2022videomae,bertasius2021spaceTimesformer,wang2023videomaev2}. In such methods, carefully designed pretext tasks (\textit{e.g.}, frame reconstruction, temporal prediction, or masked completion) are used to capture spatio-temporal consistency without human annotations, thereby substantially mitigating the dependence on scarce high-quality labels.
Endoscopic video analysis plays a crucial role in the early screening and diagnosis of gastrointestinal diseases by facilitating more accurate lesion detection and assisting clinicians in making timely decisions. However, its further advancement is significantly hindered by the scarcity of high-quality annotated data, which limits the performance and generalization capabilities of current algorithms. 
To address this challenge, a promising strategy involves leveraging advancements in general video understanding to learn generalizable representations from large-scale unlabeled videos through self-supervised video pre-training \cite{tong2022videomae,bertasius2021spaceTimesformer,wang2023videomaev2}.
In these methods, carefully designed pretext tasks (\textit{e.g.}, frame reconstruction, temporal prediction, or masked completion) are employed to capture spatio-temporal consistency without relying on human annotations, thereby substantially reducing dependence on limited high-quality labels.


% Most existing self-supervised video pre-training methods are developed on natural videos, where the central idea is to learn semantics through dense spatio-temporal modeling, which has proven to be highly effective in tasks such as action recognition \cite{tong2022videomae,bertasius2021spaceTimesformer,wang2023videomaev2}. However, natural and endoscopic videos differ fundamentally in their semantic structures, the former rely heavily on prominent temporal dynamics to capture motion semantics and contextual evolution, whereas the latter primarily derive semantics from static, localized, and structured visual cues \cite{ji2022videopolyp}. Consequently, when existing methods  \cite{hu2024mmcrl,tian2025endomamba,wang2025improvingEndoFM-LV,wang2023foundationEndoFM} continue to adopt dense spatio-temporal modeling paradigms, a contradiction arises that models tend to fit non-semantic motions such as camera jitter and tissue displacement while neglecting truly critical static semantics like lesion morphology, color, and texture \cite{ji2022videopolyp}. This leads to a characteristic motion bias (Figure {\hypersetup{linkcolor=red}\ref{fig:introfig}}), where the model overemphasizes task-irrelevant dynamic features, thus weakening semantic focus and cross-task generalization capability \cite{ali2021deependoscopy,ji2022videopolyp}.

% However, most existing self-supervised video pre-training methods are developed on natural videos, where the core idea is to learn semantics through dense spatio-temporal modeling, which has proved highly effective for tasks such as action recognition \cite{tong2022videomae,bertasius2021spaceTimesformer,wang2023videomaev2}. Yet natural and endoscopic videos differ fundamentally in their semantic structures: the former relies heavily on prominent temporal dynamics to capture motion semantics and contextual evolution, whereas the latter primarily derives semantics from static, localized, and highly structured visual cues \cite{ji2022videopolyp}, making a direct transfer of these methods to the endoscopic domain far from optimal. When such dense spatio-temporal paradigms are directly transferred to endoscopic videos \cite{hu2024mmcrl,tian2025endomamba,wang2025improvingEndoFM-LV,wang2023foundationEndoFM,ali2021deependoscopy,ji2022videopolyp}, an inherent contradiction emerges that models tend to fit non-semantic motions such as camera jitter and tissue displacement while underutilizing truly critical static semantics like lesion morphology, color and texture \cite{ji2022videopolyp,jinhao2024PSTUDA}. We refer to this systematic tendency to overemphasize task-irrelevant dynamic patterns and underemphasize diagnostically meaningful static cues as motion bias, which ultimately weakens semantic focus and thereby degrades cross-task generalization capability.
At present, most of the existing self-supervised video pre-training methods are developed on natural videos, and their core idea is to learn semantics through dense spatio-temporal modeling, which has proven highly effective for tasks such as action recognition \cite{tong2022videomae,bertasius2021spaceTimesformer,wang2023videomaev2}. 
However, there are fundamental differences between natural and endoscopic videos in terms of their semantic structures. Natural videos heavily rely on prominent temporal dynamics to capture motion semantics and contextual evolution. In contrast, endoscopic videos primarily derive semantics from static, localized, and highly structured visual cues \cite{ji2022videopolyp}. 
% This disparity makes a direct transfer of these methodologies to the endoscopic domain suboptimal. 
Therefore, when dense spatio-temporal paradigms are directly applied to endoscopic videos \cite{hu2024mmcrl,tian2025endomamba,wang2025improvingEndoFM-LV,wang2023foundationEndoFM,ali2021deependoscopy,ji2022videopolyp}, an inherent contradiction arises: models tend to focus on non-semantic motions such as camera jitter and tissue displacement while underutilizing critical static semantics like the morphology, color, and texture of the lesion \cite{ji2022videopolyp,jinhao2024PSTUDA}.
We refer to this systematic tendency to overemphasize task-independent dynamic patterns while underestimating static cues of diagnostic significance as “motion bias”, which ultimately weakens semantic focus and thereby reduces cross-task generalization ability.

% Existing studies attempt to mitigate this bias via sparse sampling \cite{gupta2023siameseMAE,pei2024videomac,liu2025futureTCoRe}, temporal masking \cite{tong2022videomae,wang2023videomaev2}, or local attention mechanisms \cite{bertasius2021spaceTimesformer}. However, these methods still rely on motion modeling as the principal feature extraction pathway and lack explicit modeling of the semantic structural characteristics unique to endoscopic videos. This discrepancy reflects a deeper issue that the goal of endoscopic video analysis is not to pursue increasingly complex spatio-temporal modeling, but rather to develop a cognition-inspired representation learning mechanism that aligns with human perceptual principles.

% Although this motion bias can be partially alleviated by strategies such as sparse sampling \cite{gupta2023siameseMAE,pei2024videomac,liu2025futureTCoRe}, temporal masking \cite{tong2022videomae,wang2023videomaev2}, and local attention mechanisms \cite{bertasius2021spaceTimesformer}, these techniques were originally proposed for natural-video tasks such as action recognition, with the primary goal of improving efficiency and robustness of temporal modeling rather than explicitly correcting motion bias. Consequently, they still lack an explicit modeling paradigm tailored to the static, localized, and structured semantic characteristics that dominate endoscopic videos, leaving a substantial gap for further exploration.
Although this motion bias can be partially mitigated through strategies such as sparse sampling \cite{gupta2023siameseMAE,pei2024videomac,liu2025futureTCoRe}, temporal masking \cite{tong2022videomae,wang2023videomaev2}, and local attention mechanisms \cite{bertasius2021spaceTimesformer}, it is important to note that these techniques were originally developed for natural video tasks like action recognition. Their primary objective was to enhance the efficiency and robustness of temporal modeling rather than explicitly addressing motion bias. As a result, there remains a significant gap in the explicit modeling paradigms specifically designed to accommodate the static, localized, and structured semantic characteristics prevalent in endoscopic videos, warranting further investigation.

% Experienced clinicians, when examining endoscopic videos, typically first focus on semantically salient regions within individual frames—such as anomalies in color, texture, or boundary—and then assess their temporal evolution to infer lesion properties \cite{hirsch2023selfendoscopic}. This “focus before perception” observation pattern inspires our research. Following this paradigm, we propose a \textbf{F}ocus-to-\textbf{P}erceive \textbf{R}epresentation \textbf{L}earning (\textbf{\textit{FPRL}}) framework for endoscopic video analysis, aiming to fundamentally alleviate motion bias and enhance spatio-temporal semantic coordination through a semantics-driven hierarchical modeling mechanism.

% In routine clinical practice, experienced endoscopists do not rely primarily on motion to interpret endoscopic videos. Rather, they typically begin by carefully examining individual frames to identify semantically salient regions such as subtle anomalies in color, texture, or lesion boundaries before tracing the temporal evolution of these candidate regions to infer pathological characteristics \cite{hirsch2023selfendoscopic}. This process can be summarized as first focusing on diagnostically meaningful static cues, then perceiving their changes over time, while largely disregarding irrelevant motions like camera jitter or tissue displacement. Inspired by this “focus before perception” cognitive pattern, we propose \textbf{F}ocus-to-\textbf{P}erceive \textbf{R}epresentation \textbf{L}earning (\textbf{\textit{FPRL}}), a novel framework for endoscopic video analysis. \textit{FPRL} implements a semantics-driven hierarchical modeling mechanism that enhances spatio-temporal semantic coordination, thus effectively mitigating motion bias and improving representation learning (see Fig.~{\hypersetup{linkcolor=red}\ref{fig:introfig}}).
In clinical practice, experienced endoscopists do not primarily rely on motion to interpret endoscopic videos. Instead, they typically begin by meticulously examining individual frames to identify semantically salient regions, such as subtle anomalies in color, texture, or lesion boundaries. This initial analysis is followed by tracing the temporal evolution of these candidate regions to infer pathological characteristics \cite{hirsch2023selfendoscopic}. This process can be summarized as first focusing on diagnostically meaningful static cues and then perceiving their changes over time while largely disregarding irrelevant motions such as camera jitter or tissue displacement. 
Inspired by the cognitive pattern of “focus before perception”, we propose \textbf{F}ocus-to-\textbf{P}erceive \textbf{R}epresentation \textbf{L}earning (\textbf{\textit{FPRL}}), a novel framework for endoscopic video analysis. The \textit{FPRL} framework employs a semantics-driven hierarchical modeling mechanism that enhances spatio-temporal semantic coordination, effectively mitigating motion bias and improving representation learning (see Fig.~\ref{fig:introfig}).

% Specifically, our proposed \textit{FPRL} framework performs hierarchical semantic modeling by explicitly disentangling and jointly learning both static and contextual semantics.
% First, we propose a teacher-prior adaptive masking (TPAM) strategy with multi-view sparse sampling to counteract pervasive low-level dynamic noise and non-semantic motion in endoscopic videos. This suppresses redundant temporal dependencies and enhances lesion-centric semantic saliency, thereby yielding a more motion-robust static representation.
% Second, we utilize cross-view masked feature completion (CVMFC) and attention-guided temporal prediction (AGTP) to capture the temporal evolution and correlation of semantic regions. This ensures robust inter-frame semantic consistency and global contextual integrity.
% Through this semantics-driven hierarchy, \textit{FPRL} refines semantic extraction while maintaining temporal awareness, thus effectively mitigating motion bias and significantly boosting representation generalization. This work establishes a novel, cognition-inspired paradigm for endoscopic video pre-training.
Specifically, our proposed \textit{FPRL} framework performs hierarchical semantic modeling by explicitly disentangling and jointly learning both static and contextual semantics. First, we introduce a teacher-prior adaptive masking (TPAM) strategy combined with multi-view sparse sampling to suppress redundant temporal dependencies and accentuate lesion-related semantic saliency. This process effectively counteracts low-level dynamic noise and non-semantic motion, yielding a robust static representation. Subsequently, we employ the cross-view masked feature completion (CVMFC) and attention-guided temporal prediction (AGTP) to model the temporal evolution and structural correlation of semantic regions. This process establishes consistent inter-frame semantics and preserves global contextual integrity, thereby capturing coherent dynamic patterns. Through this semantics-driven hierarchical approach, \textit{FPRL} enhances semantic discriminability while retaining temporal coherence, thus substantially alleviating motion bias and improving generalization across downstream tasks. The framework establishes an innovative, cognition-inspired paradigm for endoscopic video representation learning.


% In summary, our main contributions are as follows:
% \begin{itemize}
%     \item We propose \textit{FPRL}, a cognition-inspired framework for endoscopic video analysis that learn separately static semantics and contextual semantics via a hierarchical semantic modeling mechanism, thus mitigating motion bias and yielding robust semantic refinement.
%     \item Our approach leverages \textit{teacher-prior adaptive masking} to focus on static, lesion-related local semantics, while employing \textit{cross-view masked feature completion} and \textit{attention-guided temporal prediction} to enforce the temporal continuity and global integrity of contextual semantics.
%     \item We conduct extensive experiments on 11 endoscopic video datasets and show that \textit{FPRL} consistently outperforms existing methods across diverse downstream tasks including classification, segmentation, detection, and recognition, demonstrating its effectiveness and strong generalization in endoscopic video representation learning.
% \end{itemize}
% In summary, the main contributions of this work are as follows:
In summary, our main contributions are as follows:
\begin{itemize}
    \item We are the first to develop \textit{FPRL}, a cognition-inspired representation learning framework that employs a hierarchical semantic modeling mechanism to separate and jointly learn static and contextual semantics, thereby mitigating motion bias and achieving robust representations for endoscopic video analysis.
    \item We propose a \textit{teacher-prior adaptive masking} strategy to emphasize lesion-centric static semantics, and combine it with \textit{cross-view masked feature completion} and \textit{attention-guided temporal prediction} to ensure temporal coherence and global integrity of contextual semantics.
    \item Extensive experiments conducted on 11 endoscopic video datasets show that \textit{FPRL} consistently outperforms existing methods across diverse downstream tasks including classification, segmentation, detection, and recognition, demonstrating its effectiveness and strong generalization in endoscopic video representation learning.
\end{itemize}


==> sec/2_related.tex <==
\section{Related Work}
\label{sec:related}


\subsection{Self-supervised Video Representation Learning}

% Self-supervised learning (SSL) \cite{yuzhang2025confusiondriven,he2022MAE,grill2020BYOL} leverages the inherent structure of data to generate supervisory signals, enabling the learning of transferable feature representations without manual annotation. Mainstream self-supervised video learning approaches can be broadly grouped into three categories: 1) discriminative methods that exploit temporal consistency or contrastive learning \cite{jenni2021timeCorrespendence1,qian2021timeCorrespendence2,sermanet2018timeCorrespendence3,qing2023hierarchicalconsistency}, 2) reconstruction-based masked modeling techniques, such as MVM/MFM \cite{tong2022videomae,wang2023videomaev2,liu2025futureTCoRe} and 3) the recently emerging joint embedding predictive architecture (JEPA) paradigm \cite{bardes2024vjepa}, which performs prediction directly in the representation space. 
% Self-supervised learning (SSL) \cite{yuzhang2025confusiondriven,he2022MAE,grill2020BYOL} leverages the inherent structure of data to generate supervisory signals, enabling the learning of transferable feature representations without manual annotation. Mainstream self-supervised video learning approaches primarily include discriminative methods that exploit temporal consistency or contrastive learning \cite{jenni2021timeCorrespendence1,qian2021timeCorrespendence2,sermanet2018timeCorrespendence3,qing2023hierarchicalconsistency}, reconstruction-based masked modeling techniques such as MVM/MFM \cite{tong2022videomae,wang2023videomaev2,liu2025futureTCoRe}, and the emerging joint embedding predictive architecture (JEPA) paradigm \cite{bardes2024vjepa}, which performs prediction directly in the representation space.
Self-supervised learning (SSL) \cite{yuzhang2025confusiondriven,he2022MAE,grill2020BYOL} utilizes the intrinsic structure of data to generate supervisory signals, thereby facilitating the acquisition of transferable feature representations without the need for manual annotation. The predominant approaches in self-supervised video learning encompass discriminative methods that leverage temporal consistency or contrastive learning \cite{jenni2021timeCorrespendence1,qian2021timeCorrespendence2,sermanet2018timeCorrespendence3,qing2023hierarchicalconsistency}, reconstruction-based masked modeling techniques such as MVM/MFM \cite{tong2022videomae,wang2023videomaev2,liu2025futureTCoRe}, and the emerging joint embedding predictive architecture paradigm \cite{bardes2024vjepa}, which conducts predictions directly within the representation space.


% Early self-supervised video methods primarily attempted to directly transfer image-based pretext tasks to video sequences, for instance, predicting frame order \cite{lee2017shuffleFrame2,misra2016shuffleFrame}, playback speed \cite{benaim2020speednet}, or future frames \cite{srivastava2015PredictFuture} to capture temporal dependencies. These methods were grounded in the premise that motion conveys semantic information, underscoring the importance of capturing dynamic patterns for video understanding. With the rise of the contrastive learning paradigm \cite{caron2021DINO,oquab2023dinov2,chen2020SimCLR,grill2020BYOL}, research attention shifted toward leveraging inter-sample consistency to learn spatio-temporal representations \cite{jenni2021timeCorrespendence1,qian2021timeCorrespendence2,sermanet2018timeCorrespendence3}. These techniques construct positive and negative pairs based on temporal continuity, semantic similarity, or motion cues, and have shown strong performance in discriminative tasks, leading to notable advances in downstream applications including action recognition \cite{actionrec2021large-scale,kuehne2011motionrec} and video retrieval \cite{liu2024retrieval,kordopatis2019retrieval}.

% Methods inspired by masked autoencoders \cite{he2022MAE} capture visual co-occurrence patterns by reconstructing randomly masked portions of the input, leveraging local contextual relationships. Representative approaches such as VideoMAE \cite{tong2022videomae}, VideoMAE V2 \cite{wang2023videomaev2}, and ST-MAE \cite{feichtenhofer2022ST-MAE} successfully extend masked image modeling to the video domain, adopting various masking strategies to handle the spatio-temporal redundancy present in video data. To further address the high degree of redundancy, subsequent research has explored motion-guided adaptive masking \cite{fan2023motionMGMAE,bandara2023adamae}, sparse sampling \cite{pei2024videomac,gupta2023siameseMAE,hernandez2024vicmae,liu2025futureTCoRe}, and latent-space reconstruction \cite{bardes2024vjepa} with the goal of improving semantic emphasis and training efficiency.
Early self-supervised video methods mainly transferred image-based pretext tasks to video sequences, such as predicting frame order \cite{lee2017shuffleFrame2,misra2016shuffleFrame}, playback speed \cite{benaim2020speednet}, or future frames \cite{srivastava2015PredictFuture} to capture temporal dependencies, assuming motion conveys semantic information. With the rise of the contrastive learning paradigm \cite{caron2021DINO,oquab2023dinov2,chen2020SimCLR,grill2020BYOL}, the research focus shifted to leveraging inter-sample consistency to learn spatio-temporal representations \cite{jenni2021timeCorrespendence1,qian2021timeCorrespendence2,sermanet2018timeCorrespendence3}. These techniques construct positive and negative pairs using temporal continuity, semantic similarity, or motion cues, achieving notable advances in downstream tasks such as action recognition \cite{actionrec2021large-scale,kuehne2011motionrec} and video retrieval \cite{liu2024retrieval,kordopatis2019retrieval}. 
Alternatively, methods inspired by masked autoencoders \cite{he2022MAE} learn visual co-occurrence patterns by reconstructing randomly masked portions of the input. Representative approaches like VideoMAE \cite{tong2022videomae}, VideoMAE V2 \cite{wang2023videomaev2}, and ST-MAE \cite{feichtenhofer2022ST-MAE} successfully extend masked image modeling to video with various spatio-temporal masking strategies. To further address high video redundancy, subsequent works have explored motion-guided adaptive masking \cite{fan2023motionMGMAE,bandara2023adamae}, sparse sampling \cite{pei2024videomac,gupta2023siameseMAE,hernandez2024vicmae,liu2025futureTCoRe}, and latent-space reconstruction \cite{bardes2024vjepa} for improved semantic emphasis and training efficiency.

% Overall, these approaches share the core assumption that video semantics are encoded in temporal dynamics, making dense spatiotemporal modeling sufficient for learning consistency in natural videos where action semantics correlate with motion variations.
Overall, these approaches share a fundamental assumption that the semantics of video content are encoded within temporal dynamics. This perspective renders dense spatiotemporal modeling adequate for capturing consistency in natural videos, where the semantics of actions correlate with variations in motion.

\subsection{Self-supervised Learning for Endoscopic Video}

% In endoscopic video analysis, SSL is increasingly adopted to mitigate annotation scarcity. Early studies mainly adopted lightweight pretext tasks or contrastive objectives \cite{hirsch2023selfendoscopic,vats2021endossl3,intrator2023endossl,mohammed2020endossl2} to learn discriminative representations from spatiotemporal augmentations, yielding initial gains on recognition and retrieval. 
In endoscopic video analysis, SSL addresses the challenge of annotation scarcity by learning from unlabeled data. Early approaches employed contrastive or pretext tasks \cite{hirsch2023selfendoscopic,vats2021endossl3,intrator2023endossl,mohammed2020endossl2} with spatio-temporal augmentations, achieving initial improvements in recognition and retrieval tasks.
% Building on advances in natural video SSL, recent endoscopic video research has imported similar principles. Representative efforts include EndoFM \cite{wang2023foundationEndoFM} and its long-video variant EndoFM-LV \cite{wang2025improvingEndoFM-LV}. They use contrastive objectives to enforce consistency across spatio-temporal views. EndoFM-LV further scales pret-raining to minute level sequences and conducts training on 32-frame clips, which improves temporal robustness. Meanwhile, M$^2$CRL \cite{hu2024mmcrl} systematically introduces the masked modeling paradigm into endoscopic video analysis, employing both spatial and temporal masking strategies to improve contextual reconstruction and structural semantic learning. More recently, EndoMamba \cite{tian2025endomamba} explores long-sequence modeling based on the Mamba architecture \cite{gu2024mamba,gu2022S4,gu2020hippo,liu2024vmamba,li2024videomamba,zhu2024visionmamba} and employs the hierarchical pre-training paradigm to decouple high-level and low-level semantics.
% Recent methods adapt advances from natural video SSL. EndoFM \cite{wang2023foundationEndoFM} and EndoFM-LV \cite{wang2025improvingEndoFM-LV} apply contrastive learning across spatio-temporal views, with the latter extending to minute-level sequences for enhanced temporal modeling. Meanwhile, M$^2$CRL \cite{hu2024mmcrl} introduces masked modeling using spatial and temporal masking to improve contextual reconstruction. EndoMamba \cite{tian2025endomamba} further explores long-sequence modeling via Mamba architecture \cite{gu2024mamba,gu2022S4,gu2020hippo,liu2024vmamba,zhu2024visionmamba} with hierarchical pretraining to separate high-level and low-level semantics.
Recent approaches have adapted innovations from natural video SSL. EndoFM \cite{wang2023foundationEndoFM} and EndoFM-LV \cite{wang2025improvingEndoFM-LV} implement contrastive learning across spatio-temporal views, with the latter extending to minute-level sequences to enhance temporal modeling capabilities. Concurrently, M$^2$CRL \cite{hu2024mmcrl} introduces masked modeling techniques that utilize both spatial and temporal masking to improve contextual reconstruction. Furthermore, EndoMamba \cite{tian2025endomamba} delves into long-sequence modeling through the Mamba architecture \cite{gu2024mamba,gu2022S4,gu2020hippo,liu2024vmamba,zhu2024visionmamba}, incorporating hierarchical pretraining to differentiate between high-level and low-level semantics.

% Despite these advances, the prevailing motion-dominant assumption remains prevalent. This is problematic for endoscopic video analysis, where semantics depend fundamentally on static, localized, and structured visual cues such as lesion morphology, color, and texture \cite{ji2022videopolyp}, rather than motion. Consequently, models trained under motion-centered objectives tend to overfit non-semantic motions (\textit{e.g.}, camera jitter or tissue displacement) while failing to adequately represent the static features essential for diagnosis \cite{ali2021deependoscopy,ji2022videopolyp}.
% However, these methods predominantly follow the motion-centric assumption, which is problematic for endoscopic analysis where diagnostic semantics primarily rely on static morphological features like lesion color and texture \cite{ji2022videopolyp}. Consequently, motion-focused objectives often overfit to non-semantic artifacts (e.g., camera jitter, tissue movement) while underrepresenting crucial static features for diagnosis \cite{ali2021deependoscopy,ji2022videopolyp}.
Nevertheless, these methods predominantly adhere to a motion-centric paradigm, which poses significant challenges for endoscopic analysis where diagnostic semantics are primarily dependent on static morphological features such as the color and texture of the lesion \cite{ji2022videopolyp}. As a result, motion-focused objectives often overfit non-semantic artifacts (\textit{e.g.}, camera jitter or tissue displacement), while inadequately representing critical static features essential for accurate diagnosis \cite{ali2021deependoscopy,ji2022videopolyp}.



\subsection{Hierarchical Representation Learning}

% Recent advances in self-supervised video learning are increasingly focused on hierarchical representation learning \cite{xiao2022hierarchicalsep,qing2023hierarchicalconsistency}. This approach aims to disentangle complementary semantic cues by organizing video information into multi-level abstractions, typically separating static spatial semantics from dynamic temporal context to produce structured and interpretable representations.
% Recent self-supervised video learning increasingly focuses on hierarchical representation learning \cite{xiao2022hierarchicalsep,qing2023hierarchicalconsistency}, which disentangles complementary semantic cues by organizing video content into multi-level abstractions, which typically separating static spatial semantics from dynamic temporal context, to yield structured and interpretable representations.
Recent advancements in self-supervised video learning have increasingly emphasized hierarchical representation learning \cite{xiao2022hierarchicalsep,qing2023hierarchicalconsistency}. This approach effectively disentangles complementary semantic cues by organizing video content into multi-level abstractions, typically distinguishing static spatial semantics from dynamic temporal contexts, to yield structured and interpretable representations. 

% In general video domains, hierarchical modeling has been explored through strategies such as spatio–temporal disentanglement \cite{wang2015stsep,diba2018stsep2,qing2023stsep3,korbar2019stsep4}, multi-stage or cross-scale encoding \cite{liu2022multisep2,arnab2021vivitmultisep}, and masked hierarchical reconstruction \cite{feichtenhofer2022ST-MAE,wang2023videomaev2,xiao2022hierarchicalsep,reed2023scalesep}. These approaches demonstrate that hierarchical architectures can effectively capture both fine-grained appearance details and long-range temporal dependencies, leading to improved generalization and efficiency over flat-structured models. In contrast, such strategies remain largely underexplored in the context of endoscopic video analysis. Existing pre-training frameworks still model spatial and temporal information in a tightly coupled manner. This overlooks a critical aspect of endoscopic semantics that diagnostically meaningful cues emerge from structured spatial patterns and their distinct temporal evolution, which are not adequately captured by non-hierarchical modeling methods.
% In general video domains, hierarchical modeling has been explored via spatio-temporal disentanglement \cite{wang2015stsep,diba2018stsep2,qing2023stsep3,korbar2019stsep4}, multi-stage or cross-scale encoding \cite{liu2022multisep2,arnab2021vivitmultisep}, and masked hierarchical reconstruction \cite{feichtenhofer2022ST-MAE,wang2023videomaev2,xiao2022hierarchicalsep,reed2023scalesep}. These strategies capture both fine-grained appearance and long-range temporal dependencies, improving generalization and efficiency over flat models. However, such hierarchical approaches remain largely unexplored in endoscopic video analysis, where existing methods still model spatial and temporal information jointly. This overlooks a key endoscopic characteristic that diagnostic semantics arise from structured spatial patterns and their temporal evolution, which are inadequately captured by non-hierarchical modeling.
In general video domains, hierarchical modeling has been investigated through various methods including spatio-temporal disentanglement \cite{wang2015stsep,diba2018stsep2,qing2023stsep3,korbar2019stsep4}, multi-stage or cross-scale encoding \cite{liu2022multisep2,arnab2021vivitmultisep}, and masked hierarchical reconstruction \cite{feichtenhofer2022ST-MAE,wang2023videomaev2,xiao2022hierarchicalsep,reed2023scalesep}. These strategies are adept at capturing both fine-grained appearance details and long-range temporal dependencies, thereby enhancing generalization and efficiency compared to flat models. However, such hierarchical approaches remain largely underexplored in the context of endoscopic video analysis. Existing methodologies continue to model spatial and temporal information jointly. This overlooks a key endoscopic characteristic that diagnostic semantics arise from structured spatial patterns and their temporal evolution, which are inadequately captured by non-hierarchical modeling.

% To bridge this gap, we propose \textbf{F}ocus-to-\textbf{P}erceive \textbf{R}epresentation \textbf{L}earning (\textbf{\textit{FPRL}}), a hierarchical pre-training framework that explicitly factorizes endoscopic video representations into static appearance semantics and temporal contextual semantics, enhancing the capture of diagnostic cues and boosting downstream analysis performance.




==> sec/3_method.tex <==
\section{Methodology}
\label{sec:method}


\begin{figure*}
    \centering
    \includegraphics[width=1\linewidth]{FPRL.png}
    \caption{The pipeline of the proposed \textit{FPRL}. For static semantic focus, we employ a teacher-prior adaptive masking strategy coupled with pixel reconstruction. For contextual semantic perception, we use cross-view masked feature completion with latent spatial alignment and an attention-guided temporal prediction module with contrastive learning.}
    \label{fig:FPRL}
\end{figure*}

\subsection{Overview}

As illustrated in Fig. \ref{fig:FPRL}, our proposed \textit{FPRL} is a cognition-inspired hierarchical framework that emulates the clinical examination process of endoscopic videos. 
The aim is first to focus on lesion-centric salient representations and then to enforce cross-view consistency via feature correlation. 
In order to operationalize this cognitive process, we propose a hierarchical semantic modeling mechanism, which consists of two components: \textit{Static Semantic Focus} and \textit{Contextual Semantic Perception}. 
The former is used to capture lesion-centered intra-view semantics, and the latter is employed to model cross-view temporal evolution to maintain contextual consistency. 
This hierarchy refines semantics and explicitly mitigates the motion bias common in endoscopic videos.

To suppress low-level dynamic noise and non-semantic motion, we develop the Teacher-Prior Adaptive Masking (TPAM) based on multi-view sparse sampling in Section \ref{3.2}, which uses teacher-derived saliency features to guide students to find lesion-centered local cues to produce robust static representations. 
We then enhance inter-frame semantic consistency and global contextual integrity by the Cross-View Masked Feature Completion (CVMFC) and Attention-Guided Temporal Prediction (AGTP) in Section \ref{3.3}. 
Finally, we optimize a unified objective in Section \ref{3.4} that combines pixel-wise reconstruction, feature alignment, and temporal prediction loss to enable collaborative learning of static and contextual semantics and produce temporally consistent representations.

% In Section \ref{3.2}, we address the low-level dynamic noise and non-semantic motion prevalent in endoscopic videos by introducing multi-view sparse sampling and a \textit{Teacher-Prior Adaptive Masking} (TPAM) mechanism. The former provides diverse frame views to suppress redundant temporal dependencies among consecutive frames, while the latter leverages teacher-provided semantic saliency to guide the student toward lesion-related local semantics, yielding robust static semantics.

% In Section \ref{3.3}, we further capture cross-frame semantic correspondence and structured temporal evolution through two submodules: \textit{Cross-View Masked Feature Completion} (CVMFC) and \textit{Attention-Guided Temporal Prediction} (AGTP). CVMFC retrieves and completes masked semantic information from features across temporal views to ensure inter-frame semantic consistency and cross-view alignment, whereas AGTP aggregates salient regional features to model inter-frame evolution, enforcing temporal semantic continuity and global contextual integrity.

% Finally, in Section \ref{3.4}, we jointly optimize pixel-level reconstruction, cross-view feature alignment, and temporal prediction objectives to enable collaborative learning of static semantics and contextual semantics. This unified objective harmonizes semantic refinement with temporally consistent contextual perception.




\subsection{Semantic Focus for Static Representation}
\label{3.2}

To obtain robust intra-view semantics in the presence of non-semantic motion, we propose \textit{Static Semantic Focus}, which concentrates modeling capacity on lesion-centric cues while suppressing redundant temporal correlations introduced by camera jitter and tissue motion. This design produces stable static representations that serve as a reliable anchor for subsequent cross-view modeling.


% -------------------------------------------------------------
% \paragraph{Multi-view Sparse Sampling.}
\noindent\textbf{Multi-view Sparse Sampling.} Given a video sequence 
\(
V = \{F_t \in \mathbb{R}^{H \times W \times C}\}_{t=1}^{T},
\)
we randomly select a temporal window 
\(
\mathcal{W} = [t_a, t_b]
\)
and independently sample three sparse views (past, current, and future) without replacement:
\begin{equation}
\mathcal{V}_{\text{p}},~ \mathcal{V}_{\text{c}},~ \mathcal{V}_{\text{f}} \subset \mathcal{W},
\quad 
|\mathcal{V}_{\text{p}}| = |\mathcal{V}_{\text{c}}| = |\mathcal{V}_{\text{f}}| = 2,
\end{equation}

This sampling strategy intuitively suppresses the dynamic redundancy of video input while maintaining semantic diversity across views.
Each view $\mathcal{V}$ is partitioned into non-overlapping patches and linearly embedded into a token sequence:
\begin{equation}
X = \mathrm{Embed}(\mathcal{V}) \in \mathbb{R}^{N \times d},
\end{equation}
where \(N\) denotes the total number of tokens and \(d\) is the embedding dimension.  
We adopt a teacher–student design with the current view processed by the teacher encoder $f_t$:
\begin{equation}
z_t = f_t(X_{\!c}) \in \mathbb{R}^{N \times d},
\end{equation}
while the past and future views are encoded by the student encoder $f_s$ into $z_p$ and $z_f$, respectively. The teacher provides saliency priors and alignment targets (no gradient), and the student is trainable.


% -------------------------------------------------------------
% \paragraph{Semantic Information Extraction.}
\noindent\textbf{Semantic Information Extraction.} We build encoders upon Mamba-based blocks derived from the Selective State Space Model (SSM) \cite{gu2020hippo,gu2024mamba,gu2022S4}, which models a 1D continuous-time input $x(t)$ via a hidden state $h(t)$:
\begin{equation}
h'(t) = A h(t) + B x(t), \quad y(t) = C h(t),
\label{eq:ssm_ode}
\end{equation}
where $A \in \mathbb{R}^{r\times r}$, $B \in \mathbb{R}^{r\times 1}$, and $C \in \mathbb{R}^{1\times r}$. 
Discretization with a learnable timescale $\Delta$ leads to:
\begin{equation}
\left\{
\begin{aligned}
\overline{A} &= \exp(\Delta A),\\
\overline{B} &= (\Delta A)^{-1}\big(\exp(\Delta A) - I\big)\cdot \Delta B,
\end{aligned}
\right.
\label{eq:mamba_discrete}
\end{equation}


The hidden state is then updated recursively as 
\(h_t = \overline{A} h_{t-1} + \overline{B} x_t\), 
allowing long-range dependency modeling through state propagation while maintaining linear-time complexity.

Based on this formulation, we instantiate the student encoder $f_s$ with EndoMamba \cite{tian2025endomamba} trained from scratch, and the teacher encoder $f_t$ with a VideoMamba \cite{li2024videomamba} model pre-trained on large-scale video data (frozen during training). EndoMamba adopts a hybrid topology:
\begin{itemize}
    \item \textbf{Bidirectional Mamba} performs forward and backward state propagation within each frame’s patch sequence to capture intra-frame spatial consistency and detailed texture semantics.
    \item \textbf{Unidirectional Mamba} applies a single forward state update over all patches across frames to integrate inter-frame contextual dynamics in a temporally causal manner.
\end{itemize}

Alternating these two paths across layers yields explicit spatio-temporal decoupling: the bidirectional path stabilizes static semantics, while the unidirectional path integrates contextual dynamics. This matches \textit{FPRL}’s hierarchical semantic modeling mechanism and provides a semantic information basis for subsequent lesion-centric static representations.


% -------------------------------------------------------------
% \paragraph{Teacher-Prior Adaptive Masking.}
\noindent\textbf{Teacher-Prior Adaptive Masking.} 
To sharpen static semantic focus on the current view, we propose a Teacher-Prior Adaptive Masking (TPAM)  as shown in Fig.~\ref{fig:FPRL}(b) that fuses a teacher-derived saliency prior with a lightweight attention head on tokens, thereby selecting visually prominent, lesion-correlated patches as visible while suppressing low-saliency background tokens.

% Using the teacher feature $z_t$, we derive saliency prior $H \in \mathbb{R}^{N}$ that increases the selection probability of lesion-related tokens and regularizes the mask away from background clutter. In parallel, a lightweight multi-head self-attention module applied to $\mathcal{V}_{\text{c}}$ with a linear readout produces logits that capture complementary, image-specific saliency to calibrate the final mask.
We compute a saliency prior $H \in \mathbb{R}^{N}$ through $\ell_2$-normalization of the teacher feature $z_t$, enhancing the selection of lesion-related tokens and suppressing background clutter. In parallel, a lightweight multi-head self-attention module applied to $\mathcal{V}_{\text{c}}$ with a linear projection produces logits that capture complementary, image-specific saliency to calibrate the final mask.
% The teacher features $z_t$ are spatially aggregated to produce a saliency prior $H \in \mathbb{R}^{N}$. 
% In parallel, a lightweight attention head (embedding $\rightarrow$ MHA $\rightarrow$ linear) generates mask logits:
\begin{equation}
R = \mathrm{Linear}\!\big(\mathrm{MHA}(\mathrm{Embed}(\mathcal{V}_{\text{c}}))\big) \in \mathbb{R}^{N},
\end{equation}

We fuse the two cues and compute patch-wise sampling probabilities:
\begin{equation}
S = \alpha H + (1-\alpha) R, \qquad
P = \mathrm{Softmax}(S),
\end{equation}
where $\alpha \in [0,1]$ balances the teacher prior and the attention-derived mask logits. 
Visible patches are then selected by Top-$K$ over $P$, yielding a binary (learnable) mask $M \in \{0,1\}^{N}$ with visible index set $\Omega_v$ and masked index set $\Omega_m$.
The masked current view is fed into the student encoder to obtain the current representation:
\begin{equation}
z_c = f_s\!\big(X_{\!c}^{(\Omega_v)}\big) \in \mathbb{R}^{N \times d},
\end{equation}
where $X_{\!c}^{(\Omega_v)}$ denotes the subset of tokens selected by $M$. 
Since $P$ is parameterized by the attention head (and $\alpha$), the mask $M$ is learnable via the probabilities \cite{bandara2023adamae}, enabling TPAM to concentrate representation capacity on lesion-related local semantics while suppressing redundant background responses.


\begin{table*}[t]
\caption{Comparison with other latest SOTA methods on 3 downstream tasks. We report F1 score (\%) for PolypDiag, Dice (\%) for CVC-12k, and F1 score (\%) for KUMC, respectively.}
\small
\centering
\setlength{\tabcolsep}{10pt}
\renewcommand{\arraystretch}{1.2}
\begin{tabular}{ccccccc}
\toprule
Method              & Venue   & Year & \begin{tabular}[c]{@{}c@{}}Pretrain\\  Time(h)\end{tabular} & \begin{tabular}[c]{@{}c@{}}PolypDiag\\ (Classificaton)\end{tabular} & \begin{tabular}[c]{@{}c@{}}CVC-12k\\ (Segmentation)\end{tabular} & \begin{tabular}[c]{@{}c@{}}KUMC\\ (Detection)\end{tabular} \\ \hline
Scratch (Rand.init.) & -       & -    & N/A                                                             & 83.5 ± 1.3                                                            & 53.2 ± 3.2                                                         & 73.5 ± 4.3                                                   \\ \hline
FAME \cite{FAME}               & CVPR    & 2022 & 48.9                                                            & 85.4 ± 0.8                                                            & 67.2 ± 1.3                                                         & 76.9 ± 1.2                                                   \\
ProViCo \cite{ProViCo}            & CVPR    & 2022 & 71.2                                                            & 86.9 ± 0.5                                                            & 69.0 ± 1.5                                                         & 78.6 ± 1.7                                                   \\
VCL \cite{VCL}                & ECCV    & 2022 & 74.9                                                            & 87.6 ± 0.6                                                            & 69.1 ± 1.2                                                         & 78.1 ± 1.9                                                   \\
ST-Adapter \cite{ST-Adapter}         & NeurIPS & 2022 & 8.1                                                             & 84.8 ± 0.7                                                            & 64.3 ± 1.9                                                         & 74.9 ± 2.9                                                   \\
VideoMAE \cite{tong2022videomae}           & NeurIPS & 2022 & 25.3                                                            & 91.4 ± 0.8                                                            & 80.9 ± 1.0                                                         & 82.8 ± 1.9                                                   \\
Endo-FM \cite{wang2023foundationEndoFM}            & MICCAI  & 2023 & 20.4                                                            & 90.7 ± 0.4                                                            & 73.9 ± 1.2                                                         & 84.1 ± 1.3                                                   \\
DropMAE \cite{wu2023dropmae}            & CVPR    & 2023 & 37.9                                                            & 88.2 ± 0.8                                                            & 80.9 ± 0.3                                                         & 81.7 ± 2.6                                                   \\
VideoMAE V2 \cite{wang2023videomaev2}        & CVPR    & 2023 & 17.3                                                            & 89.6 ± 1.4                                                            & 81.0 ± 0.4                                                         & 84.2 ± 1.0                                                   \\
M$^2$CRL \cite{hu2024mmcrl}             & NeurIPS & 2024 & 24.3                                                               & 94.2 ± 0.7                                                                    & 81.4 ± 0.8                                                                 & 86.3 ± 0.8                                                             \\
VideoMamba \cite{li2024videomamba}       & ECCV    & 2024 & 55.4                                                               & 88.2 ± 0.9                                                                    & 82.8 ± 0.5                                                                  & 84.1 ± 1.0                                                             \\
EndoFM-LV \cite{wang2025improvingEndoFM-LV}         & JBHI    & 2025 & 56.1                                                               & 94.5 ± 0.4                                                                    & 82.6 ± 0.3                                                                 & 72.6 ± 1.2                                                            \\
EndoMamba \cite{tian2025endomamba}      & MICCAI  & 2025 & 38.2                                                               & 94.5 ± 0.2                                                                   & 84.5 ± 0.8                                                                 & 88.8 ± 0.1                                                            \\ 
\hline
FPRL                 & Ours    & -    & 18.2                                                            & \textbf{95.2 ± 0.3}{$\color{highlight}\textbf{\footnotesize{$\uparrow$}0.7}$}                                                   & \textbf{86.1 ± 0.1}{$\color{highlight}\textbf{\footnotesize{$\uparrow$}1.6}$}                                                & \textbf{89.8 ± 0.1}{$\color{highlight}\textbf{\footnotesize{$\uparrow$}1.0}$}                                             \\ 
\bottomrule
\end{tabular}
\label{tab:result}
\end{table*}



\subsection{Contextual Perception for Semantic Correspondence}
\label{3.3}

Building upon the static representation, we further propose \textit{Contextual Semantic Perception} to explicitly establish reliable correspondence across views and model structured inter-frame evolution. This is achieved by two dedicated submodules: Cross-View Masked Feature Completion (CVMFC) and Attention-Guided Temporal Prediction (AGTP).

% -------------------------------------------------------------
% \paragraph{Cross-View Masked Feature Completion.}
\noindent\textbf{Cross-View Masked Feature Completion.} 
As shown in Fig.~\ref{fig:FPRL}(d), CVMFC performs fine-grained correspondence in the latent space and completes the masked current stream by retrieving semantics from adjacent views. 
Given the masked current features $z_c\!\in\!\mathbb{R}^{N\times d}$ and the student features of the past and future views $z_p,z_f\!\in\!\mathbb{R}^{N\times d}$, we adopt a Transformer-style block (cross-attention $\rightarrow$ self-attention $\rightarrow$ FFN) with two symmetric paths that use $z_p$ and $z_f$ as a temporal dictionary. 
Queries are formed from the current view, while keys/values come from the adjacent views.
For example, we set queries from the current view and keys/values from the past view:
\begin{equation}
\label{eq:cvmfc_proj_p}
Q_c = z_c W_q,\qquad
K_p = z_p W_k,\qquad
V_p = z_p W_v ,
\end{equation}
and compute cross-attention:
\begin{equation}
\label{eq:cvmfc_cross_p}
z_c^{\prime}=\mathrm{Softmax}\!\left(\frac{Q_c K_p^\top}{\sqrt{d}}\right)V_p ,
\end{equation}
The result is refined by self-attention and FFN:
\begin{equation}
\label{eq:cvmfc_final_p}
z_c^{\prime\prime}=\mathrm{SA}(z_c^{\prime}),\qquad 
z_c^{p}=\mathrm{FFN}(z_c^{\prime\prime}) ,
\end{equation}
Similarly, the $z_c^f$ can be generated in the same manner.

Layer normalization and residual connections follow standard practice (omitted for brevity). The outputs $z_c^p$ and $z_c^f$ are separately aligned with the frozen teacher features $z_t$ of the current view in Section~\ref{3.4}. 
This module establishes cross-view correspondence in a compact latent space and preserves temporal semantic continuity at the token level.

% -------------------------------------------------------------
% \paragraph{Attention-Guided Temporal Prediction.}
\noindent\textbf{Attention-Guided Temporal Prediction.}
As shown in Fig.~\ref{fig:FPRL}(c), AGTP enforces view-level temporal correspondence consistency across different views. 
Unlike CVMFC’s token-wise retrieval, AGTP aggregates each view according to its cross-attention with the current view and compares it to a lesion-centric current representation produced by \emph{Static Semantic Focus} (Section~\ref{3.2}). 

Let $A_c^{p}\!\in\!\mathbb{R}^{N\times N}$ be the cross-attention map from the current view (queries) to the past view (keys/values) computed in CVMFC, and let $z_p=\{z_p^{(j)}\}_{j=1}^{N}$ be the past-view tokens. 
We first derive normalized pooling weights from $A_c^{p}$, then pool $z_p$, and project the pooled vector by a target head:
\begin{equation}
\label{eq:agtp_past}
\left\{
\begin{aligned}
a_p  &\,=\, \mathrm{Norm}\!\left(\tfrac{1}{N}\sum_{i=1}^{N} A_c^{p}(i,:)\right) \in \mathbb{R}^{N},\\
z_p' &\,=\, \sum_{j=1}^{N} a_p(j)\, z_p^{(j)} \in \mathbb{R}^{d},\\
p_p  &\,=\, \phi_t\!\big(z_p'\big) \in \mathbb{R}^{d'},
\end{aligned}
\right.
\end{equation}
where $\mathrm{Norm}(u)=u/(\mathbf{1}^\top u)$ ensures $\sum_j a_p(j)=1$, and $\phi_t$ is a lightweight projector (\textit{e.g.}, two linear layers with nonlinearity). 
The future view is handled symmetrically using $A_c^{f}$ and $z_f$ to obtain $p_f$.

For the current view, the visual patches revolve around the lesion-related region, so we omit attention pooling and directly project a global average over current tokens:
\begin{equation}
\label{eq:agtp_cur}
\left\{
\begin{aligned}
&\mathrm{GAP}(z_c) \,=\, \tfrac{1}{N}\sum_{i=1}^{N} z_c^{(i)} \in \mathbb{R}^{d},\\
&p_c \,=\, \phi_c\!\big(\mathrm{GAP}(z_c)\big) \in \mathbb{R}^{d'},
\end{aligned}
\right.
\end{equation}

To provide stable, non-degenerate targets, the target head is updated from the query head by EMA \cite{grill2020BYOL} with momentum $m\!\in\![0,1)$ (stop-gradient on $p_p$ and $p_f$):
\begin{equation}
\label{eq:agtp_ema}
\phi_t \;\leftarrow\; m\,\phi_t \;+\; (1{-}m)\,\phi_c,
\end{equation}

The view-level objectives using $(p_c,p_p,p_f)$ are defined in Section~\ref{3.4}.




\begin{figure*}
    \centering
    \includegraphics[width=1\linewidth]{visuals_cr.png}
    \caption{Qualitative results of segmentation and detection tasks. The segmentation results (green, red, and yellow regions represent the true positive, false positive, and false negative, respectively) on the left are from the CVC-12k dataset, while the detection results on the right are from the KUMC dataset.}
    \label{fig:qualitative}
\end{figure*}




\subsection{Pre-training Objective}
\label{3.4}

We jointly optimize three objectives to couple static semantics and contextual semantics: 
1) pixel-level reconstruction on masked current tokens to recover lesion-centric texture/boundary details and suppress low-level motion noise, 
2) cross-view feature alignment between CVMFC outputs and the frozen teacher to establish fine-grained temporal correspondence, and 
3) temporal prediction contrastive learning from AGTP to maintain temporal consistency of view-level semantics.

% \paragraph{Pixel Reconstruction.}
\noindent\textbf{Pixel Reconstruction.} Normalized pixel values are used as explicit signals to stabilize the pre-training process.
% Let $X_c$ be the tokenized current view, $\Omega_m$ the masked index set from TPAM, and $\hat{X}_c^{(\Omega_m)}$ the reconstruction from a lightweight decoder $g$ given $z_p$. 
Given the tokenized current view $X_c$, with the masked index set $\Omega_m$ from TPAM, and the reconstruction $\hat{X}_c$ from a lightweight decoder $g$ using $z_c$ as input. 
We minimize the mean squared error over masked tokens as:
\begin{equation}
\label{eq:loss_rec}
\mathcal{L}_{\mathrm{Rec}}
 \;=\; \frac{1}{|\Omega_m|}\sum_{i\in\Omega_m}
 \big\|\,\hat{X}_c^{(i)} - X_c^{(i)}\,\big\|_2^2,
\end{equation}

% \paragraph{Cross-View Feature Alignment.}
\noindent\textbf{Cross-View Feature Alignment.} CVMFC yields two updated current streams $z_c^p$ and $z_c^f$, which are aligned to the frozen teacher features $z_t$ on the current view. 
We use cosine similarity for past/future-to-teacher alignment and an $\ell_2$ consistency between the two streams for stable features completion:
\begin{equation}
\label{eq:loss_pt}
\mathcal{L}_{pt}
= 1 - \frac{1}{|\Omega_m|} \sum_{i\in\Omega_m}
\cos\!\big(z_c^{p(i)},\, z_t^{(i)}\big),
\end{equation}

\begin{equation}
\label{eq:loss_ft}
\mathcal{L}_{ft}
= 1 - \frac{1}{|\Omega_m|} \sum_{i\in\Omega_m}
\cos\!\big(z_c^{f(i)},\, z_t^{(i)}\big),
\end{equation}

\begin{equation}
\label{eq:loss_pf}
\mathcal{L}_{pf}
= \frac{1}{|\Omega_m|} \sum_{i\in\Omega_m}
\big\| z_c^{p(i)} - z_c^{f(i)} \big\|_2^2,
\end{equation}
% \begin{equation}
% \label{eq:loss_align_terms}
% \begin{aligned}
% \mathcal{L}_{pt} 
% &= 1 - \frac{1}{|\Omega_m|} \sum_{i\in\Omega_m}
% \cos\!\big(z_c^{p(i)},\, z_t^{(i)}\big),\\
% \mathcal{L}_{ft} 
% &= 1 - \frac{1}{|\Omega_m|} \sum_{i\in\Omega_m}
% \cos\!\big(z_c^{f(i)},\, z_t^{(i)}\big),\\
% \mathcal{L}_{pf} 
% &= \frac{1}{|\Omega_m|} \sum_{i\in\Omega_m}
% \big\|\, z_c^{p(i)} - z_c^{f(i)} \,\big\|_2^2.
% \end{aligned}
% \end{equation}
where 
\(\cos(u,v)=\tfrac{u^\top v}{\|u\|_2\|v\|_2}\).
The alignment loss is as follows:
\begin{equation}
\label{eq:loss_align}
\mathcal{L}_{\mathrm{Align}} \;=\; 
\mathcal{L}_{pt} \;+\; \mathcal{L}_{ft} \;+\; \lambda_{\mathrm{pf}}\, \mathcal{L}_{pf},
\end{equation}
where $\lambda_{\mathrm{pf}}$ is the scalable weight.

% \paragraph{Temporal Prediction Contrastive Learning.}
\noindent\textbf{Temporal Prediction Contrastive Learning.} AGTP produces the view-level embeddings \(p_c\), \(p_p\) and  \(p_f\). 
We adopt InfoNCE with in-batch keys, positives are \((p_c, p_p)\) and \((p_c, p_f)\), while negatives are other keys in the batch, thus the contrastive learning loss can be defined with temperature $\tau$ and key set $\mathcal{K}$ as:
\begin{equation}
\label{eq:loss_cl}
\begin{aligned}
\mathcal{L}_{\mathrm{CL}}
= &- \log \frac{\exp(\langle p_c, p_p\rangle/\tau)}
{\sum_{k\in\mathcal{K}} \mathbf{1}[k\neq p_p] \exp(\langle p_c, k\rangle/\tau)} \\
&- \log \frac{\exp(\langle p_c, p_f\rangle/\tau)}
{\sum_{k\in\mathcal{K}} \mathbf{1}[k\neq p_f] \exp(\langle p_c, k\rangle/\tau)},
\end{aligned}
\end{equation}

% \paragraph{Overall Objective.}
\noindent\textbf{Overall Objective.} The total pre-training loss is a weighted sum, which can be formulated as:
\begin{equation}
\label{eq:loss_total}
\mathcal{L}_{\mathrm{total}} 
\;=\; \lambda_{\mathrm{1}}\,\mathcal{L}_{\mathrm{Rec}}
\;+\; \lambda_{\mathrm{2}}\,\mathcal{L}_{\mathrm{Align}}
\;+\; \lambda_{\mathrm{3}}\,\mathcal{L}_{\mathrm{CL}}.
\end{equation}
where $\lambda_{\mathrm{1}}, \lambda_{\mathrm{2}}$ and $\lambda_{\mathrm{3}}$ are scalar weights. In combination, these objectives bind static, lesion-centric semantics and temporal context into a unified hierarchical representation.



==> sec/4_experiment.tex <==


\begin{table}[t]
\caption{Ablation on different components.}
\centering
\footnotesize
\renewcommand{\arraystretch}{1.25}
\setlength{\tabcolsep}{3.8pt}
\begin{adjustbox}{width=\linewidth}
\begin{tabular}{cc|ccc|ccc}
\hline
\multirow{2}{*}{$\mathcal{L}_{Rec}$} & 
\multirow{2}{*}{$\mathcal{L}_{CL}$} & 
\multicolumn{3}{c|}{$\mathcal{L}_{Align}$} & 
\multicolumn{3}{c}{Performance (\%)} \\ \cline{3-5} \cline{6-8}
 &  & $\mathcal{L}_{pt}$ & $\mathcal{L}_{ft}$ & $\mathcal{L}_{pf}$ & Cla. & Seg. & Det. \\ \hline
 &  & \checkmark &  &  & 92.3 $\pm$ 0.4 & 83.8 $\pm$ 1.1 & 84.0 $\pm$ 1.3 \\
 &  &  & \checkmark &  & 92.2 $\pm$ 0.5 & 83.5 $\pm$ 1.2 & 83.5 $\pm$ 1.7 \\
 &  & \checkmark & \checkmark &  & 94.1 $\pm$ 0.8 & 85.7 $\pm$ 1.1 & 87.3 $\pm$ 0.8 \\ 
 &  & \checkmark & \checkmark & \checkmark & 94.2 $\pm$ 0.5 & 85.5 $\pm$ 0.2 & 88.5 $\pm$ 0.3 \\
\checkmark &  &  &  &  & 92.7 $\pm$ 0.8 & 84.3 $\pm$ 0.2 & 85.4 $\pm$ 0.4 \\
 & \checkmark &  &  &  & 93.0 $\pm$ 1.4 & 79.6 $\pm$ 1.2 & 84.1 $\pm$ 1.3 \\
\checkmark &  & \checkmark & \checkmark & \checkmark  & 93.8 $\pm$ 0.5 & 85.8 $\pm$ 0.3 & 87.5 $\pm$ 0.3 \\
 & \checkmark & \checkmark & \checkmark & \checkmark  & 94.2 $\pm$ 0.4 & 84.0 $\pm$ 1.5 & 86.1 $\pm$ 0.9 \\
\rowcolor{pink!28}
\checkmark & \checkmark & \checkmark & \checkmark & \checkmark  & \textbf{95.2 $\pm$ 0.3}  & \textbf{86.1 $\pm$ 0.1}  & \textbf{89.8 $\pm$ 0.1} \\ \hline
\end{tabular}
\end{adjustbox}
\label{tab:Components}
\end{table}



\section{Experiments}
\label{sec:experiment}

% In this section, we conduct experiments to validate the effectiveness of our \textit{FPRL}. We begin with the datasets and basic settings in Sec. \ref{4.1}. Next, we provide  quantitative and qualitative comparisons on three downstream tasks in Sec. \ref{4.2}. Finally, ablation studies are shown in Sec. \ref{4.3}. Please refer to \textit{Supplementary Material} for further details.

%-------------------------------------------------------------------------
\subsection{Datasets and Experimental Settings}
\label{4.1}

\noindent{\textbf{Datasets.}} We conduct experiments on 11 publicly available endoscopic video datasets: Colonoscopic \cite{mesejo2016Colonoscopic}, SUN-SEG \cite{ji2022videopolyp}, LDPolypVideo \cite{ma2021ldpolypvideo}, Hyper-Kvasir \cite{borgli2020hyperkvasir}, Kvasir-Capsule \cite{smedsrud2021kvasir}, CholecTriplet \cite{nwoye2022CholecTriplet}, Renji-Hospital \cite{wang2023foundationEndoFM}, PolypDiag \cite{tian2022PolypDiag}, CVC-12k \cite{bernal2015CVC-12k}, KUMC \cite{li2021KUMC} and Cholec80 \cite{twinanda2016cholec80}. These comprise 33,311 videos totaling approximately 6M frames, covering 3 types of endoscopy examination protocols and 10$+$ different diseases. The videos are processed into 30fps clips with an average duration of 5 seconds.

\noindent{\textbf{Settings.}} The first 7 datasets are used for pre-training and we sample 3 views from each video where frames are resized to spatial size of 224×224 and frame number of 2 as pre-training input. We adopt EndoMamba-S \cite{tian2025endomamba} with a patch size of 16 as the backbone model in our framework. The model is trained using the AdamW optimizer with a base learning rate of 1.5e-4, a cosine learning rate schedule for
400 epochs, and a batch size of 64, with the first five epochs dedicated to linear warmup. For feature alignment, the pretrained VideoMamba-S \cite{li2024videomamba} serves as the teacher model, with the loss weight set to \(\lambda_{\mathrm{2}}\) = 0.8 and other hyper-parameters of the loss function are set as follows: \(\lambda_{\mathrm{1}}\) = 1.0, \(\lambda_{\mathrm{3}}\) =1.0, and \(\lambda_{\mathrm{pf}}\) = 20 based on preliminary experiments. We will open source the code after the paper is accepted.

\noindent{\textbf{Evaluations.}} We evaluate our framework on 4 downstream tasks: classification on PolypDiag, segmentation on CVC-12k, detection on KUMC, and recognition on Cholec80. 
% Surgical phase recognition (Cholec80) is included in the \textit{Supplementary Material} for brevity, following a standard protocol and highlighting our method's generalization to long-horizon recognition.
Surgical phase recognition (Cholec80) is provided in \textit{Section C.1 of Supplementary Material}. This experiment follows a standardized protocol and emphasizes the generalizability of our method to long-horizon recognition.

%-------------------------------------------------------------------------
\subsection{Comparison with Prior Works}
\label{4.2}

We compare our method with several recent state-of-the-art (SOTA) approaches for endoscopy video analysis. The results of these methods are taken from the comparative method of M$^2$CRL \cite{hu2024mmcrl}, including FAME \cite{FAME}, ProViCo \cite{ProViCo}, VCL \cite{VCL}, ST-Adapter \cite{ST-Adapter}, VideoMAE \cite{tong2022videomae}, Endo-FM \cite{wang2023foundationEndoFM}, DropMAE \cite{wu2023dropmae},
and VideoMAE V2 \cite{wang2023videomaev2}. Additionally, we also compare the latest methods for video self-supervised and endoscopic video representation learning: VideoMamba \cite{li2024videomamba}, EndoFM-LV \cite{wang2025improvingEndoFM-LV}, and EndoMamba \cite{tian2025endomamba}. For a fair comparison, all methods are pretrained on the same union of 7 datasets as our \textit{FPRL}. All experimental settings are referred to those documented in their original papers or in their released codes.

\noindent{\textbf{Quantitative Evaluation.}} From Table \ref{tab:result}, we can observe that our method achieves superior performance compared to SOTA methods. Notably, under the same model architecture, our \textit{FPRL} outperforms the best existing method, EndoMamba, by improving 0.7\% F1 in classification, 1.6\% Dice in segmentation, and 1.0\% F1 in detection tasks, while also reducing pre-training time by 52\%. 
% These advancements are attributed to our approach, which enhances representation learning by employing a hierarchical semantic modeling mechanism based on multi-view sparse sampling.
These advancements can be attributed to our method, which improves representation learning by introducing a hierarchical semantic modeling mechanism that utilizes multi-view sparse sampling.

\noindent{\textbf{Qualitative Evaluation.}} 
% As visualized in Fig.~\ref{fig:qualitative}, our method produces visually convincing results in both segmentation and detection tasks. For segmentation, \textit{FPRL} accurately delineates both large and small polyps, owing to the teacher-prior adaptive masking strategy that enhances focus on lesion-related regions. In detection, our method also performs robustly, readily handling challenging scenarios with complex backgrounds.
As visualized in Fig.~\ref{fig:qualitative}, our method yields visually convincing results in both segmentation and detection tasks. For segmentation, \textit{FPRL} effectively delineates polyps of varying sizes, thanks to the teacher-prior adaptive masking strategy that enhances focus on lesion-related regions. Furthermore, in detection tasks, it obtains robust performance, adeptly managing challenging scenarios characterized by complex backgrounds.



%-------------------------------------------------------------------------
\subsection{Ablation Study}
\label{4.3}



\begin{table}[t]
\caption{Ablation on different masking strategies.}
\centering
\footnotesize
\renewcommand{\arraystretch}{1.25}
\setlength{\tabcolsep}{5pt}
\begin{adjustbox}{width=\linewidth}
\begin{tabular}{ccc|ccc}
\hline
\multicolumn{3}{c|}{Masking Strategy} & \multicolumn{3}{c}{Performance (\%)} \\ \cline{1-3} \cline{4-6}
Random & Adaptive & Teacher-Prior & Cla. & Seg. & Det. \\ \hline
\checkmark &  &  & 93.8 $\pm$ 0.5 & 85.6 $\pm$ 0.9 & 87.8 $\pm$ 1.1 \\
 & \checkmark &  & 94.5 $\pm$ 0.4 & 85.6 $\pm$ 0.7 & 83.9 $\pm$ 1.0 \\
 &  & \checkmark & 93.8 $\pm$ 0.3 & 85.7 $\pm$ 0.2 & 86.7 $\pm$ 0.8 \\
\rowcolor{pink!28}
 & \checkmark & \checkmark & \textbf{95.2 $\pm$ 0.3}  & \textbf{86.1 $\pm$ 0.1}  & \textbf{89.8 $\pm$ 0.1} \\ \hline
\end{tabular}
\end{adjustbox}
\label{tab:mask_ablation}
\end{table}
\vspace{-0.5em}  % 缩小表格后的间距

\noindent{\textbf{Analysis of Components.}}
Results in rows 1-3 of Table \ref{tab:Components} reveals that latent-space feature alignment enables the student to inherit the teacher's representations. When masked completion (\(\mathcal{L}_{pt}+\mathcal{L}_{ft}\)) is applied to both paths, performance rises by roughly 1.9\%/2.0\%/3.6\% over single-path alignment. Subsequently, enforcing past–future consistency (\(\mathcal{L}_{pf}\)) further boosts 1.2\% in detection and reduces output fluctuation, leading to a more consistent reconstruction space.
% This foundation allows pixel reconstruction (\(\mathcal{L}_{\mathrm{Rec}}\)) to deliver consistent gains, which are maximized when combined with the temporal contrastive loss \((\mathcal{L}_{\mathrm{CL}}\)), together adding 1.4\%/0.3\%/2.3\%. The full objective, exceeding the best alignment-only version by 1.0\%/0.6\%/1.3\%, demonstrates that multi-view collaboration is enhanced through stable features derived from pixel reconstruction.
The consistent gains from pixel reconstruction (\(\mathcal{L}_{\mathrm{Rec}}\)) are further maximized by the temporal contrastive loss \((\mathcal{L}_{\mathrm{CL}}\)), which provides an additional performance increase of 1.4\%/0.3\%/2.3\%. This demonstrates that their combination provides the stable features needed to enhance multi-view collaboration, with the full objective exceeding the best alignment-only version by 1.0\%/0.6\%/1.3\%.

\noindent{\textbf{Masking Strategy.}}
Table \ref{tab:mask_ablation} compares different masking strategies under a fixed masking ratio. Using random masking already surpasses other leading methods in segmentation, establishing a strong baseline. While adaptive masking improves classification, its detection performance remains limited, suggesting difficulty in identifying truly relevant regions. Teacher-prior guidance aligns with this strategy, yet the best results come from combining both approaches, demonstrating that integrating both information sources enables the model to better capture lesion-related features.


\begin{table}[t]
\caption{Ablation on different mask ratios.}
\centering
\footnotesize
\renewcommand{\arraystretch}{1.0}
\setlength{\tabcolsep}{6pt}
\begin{adjustbox}{width=\linewidth}
\begin{tabular}{c|ccc}
\hline
\multirow{2}{*}{Mask Ratio (\%)} & \multicolumn{3}{c}{Performance (\%)} \\
\cline{2-4}
& Cla. & Seg. & Det. \\ \hline
70 & 93.0 $\pm$ 2.7 & 85.3 $\pm$ 0.2 & 87.3 $\pm$ 1.2 \\
75 & 94.4 $\pm$ 0.5 & 85.1 $\pm$ 0.8 & 83.7 $\pm$ 1.0 \\
80 & 95.1 $\pm$ 0.3 & 85.4 $\pm$ 0.2 & 86.7 $\pm$ 0.9 \\
85 & 94.5 $\pm$ 0.6 & 85.5 $\pm$ 0.2 & 86.7 $\pm$ 0.7 \\
\rowcolor{pink!28}
90 & \textbf{95.2 $\pm$ 0.3}  & \textbf{86.1 $\pm$ 0.1}  & \textbf{89.8 $\pm$ 0.1} \\
95 & 92.7 $\pm$ 0.4 & 78.5 $\pm$ 1.4 & 87.1 $\pm$ 1.5 \\ \hline
\end{tabular}
\end{adjustbox}
\label{tab:mask_ratio}
\end{table}



\begin{table}[t]
\caption{Ablation on AGTP module configurations.}
\centering
\footnotesize
\renewcommand{\arraystretch}{1.2}
\setlength{\tabcolsep}{5.2pt}
\begin{adjustbox}{width=\linewidth}
\begin{tabular}{cc|ccc}
\hline
\multicolumn{2}{c|}{AGTP Configuration} & \multicolumn{3}{c}{Performance (\%)} \\ \cline{1-2} \cline{3-5}
Attn Pool & EMA Update & Cla. & Seg. & Det. \\ \hline
 &  & 93.0 $\pm$ 0.6 & 86.0 $\pm$ 0.3 & 86.9 $\pm$ 0.2 \\   
\checkmark &  & 95.0 $\pm$ 0.5 & 86.0 $\pm$ 0.1 & 86.4 $\pm$ 0.1 \\   
 & \checkmark & 95.2 $\pm$ 0.4 & 86.0 $\pm$ 0.3 & 87.7 $\pm$ 0.1 \\
\rowcolor{pink!28}   
\checkmark & \checkmark & \textbf{95.2 $\pm$ 0.3}  & \textbf{86.1 $\pm$ 0.1}  & \textbf{89.8 $\pm$ 0.1} \\  
\hline
\end{tabular}
\end{adjustbox}
\label{tab:agtp_ablation}
\end{table}


\noindent{\textbf{Masking Ratio.}}
Table~\ref{tab:mask_ratio} summarizes the impact of varying masking ratios. We can observe that as the ratio increases from 70\% to 90\%, performance across the three downstream tasks fluctuates slightly but generally improves. The increased masking encourages the model to learn more effectively from fewer visible patches, thereby enhancing its ability to capture temporal correspondences. However, at an extreme ratio of 95\%, the limited visible context hinders learning, leading to suboptimal results.

\noindent{\textbf{AGTP Configurations.}}
Our AGTP module implements temporal contrastive learning by deriving view-level features from pooled patch tokens. Within this module, attention pooling highlights salient regions, while EMA updating stabilizes the learning of representations. As presented in Table~\ref{tab:agtp_ablation}, combining both mechanisms yields the most significant gains for contrastive learning. Please refer to \textit{Section C.2 of Supplementary Material} for more ablation analyses.

% \noindent{\textbf{The Number of Sampled Frames.}}










% \begin{table}[t]
% \caption{Ablation on the number of sampled frames.}
% \centering
% \footnotesize
% \renewcommand{\arraystretch}{1.2}
% \setlength{\tabcolsep}{6pt}
% \label{tab:sample_frames}
% \begin{adjustbox}{width=\linewidth}
% \begin{tabular}{c|ccc}
% \hline
% \multirow{2}{*}{Number of Frames} & \multicolumn{3}{c}{Performance (\%)} \\
% \cline{2-4}
% & Cla. & Seg. & Det. \\ \hline
% 1 & 94.4 $\pm$ 1.6 & 86.0 $\pm$ 0.9 & 88.6 $\pm$ 1.1 \\
% \rowcolor{pink!28}
% 2 & \textbf{95.2 $pm$ 0.3}  & \textbf{86.1 $\pm$ 0.1}  & \textbf{89.8 $\pm$ 0.1} \\
% 3 & 93.0 $\pm$ 0.5 & 85.2 $\pm$ 0.4 & 85.4 $\pm$ 0.1 \\ \hline
% \end{tabular}
% \end{adjustbox}
% \end{table}

==> sec/5_conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}

In this study, we propose a cognitive framework called \textit{FPRL} for endoscopic video analysis, which employs hierarchical semantic modeling to decouple and jointly learn both static and contextual semantics. Concretely, we propose a teacher-prior adaptive masking strategy to emphasize lesion-centric regions and reduce redundant temporal dependencies. This is coupled with cross-view masked feature completion and attention-guided temporal prediction to capture structural and temporal patterns in semantic regions. Such design effectively mitigates motion bias and produces robust representations for endoscopic videos. Extensive experiments conducted on multiple publicly available datasets verify that our \textit{FPRL} consistently outperforms existing methods across diverse downstream tasks.


% \clearpage
